Adversarial Training Can Hurt Generalization

While adversarial training can improve robust accuracy (against an adversary), it sometimes hurts standard accuracy (when there is no adversary). Previous work has studied this tradeoff between standard and robust accuracy, but only in the setting where no predictor performs well on both objectives in the infinite data limit. In this paper, we show that even when the optimal predictor with infinite data performs well on both objectives, a tradeoff can still manifest itself with finite data. Furthermore, since our construction is based on a convex learning problem, we rule out optimization concerns, thus laying bare a fundamental tension between robustness and generalization. Finally, we show that robust self-training mostly eliminates this tradeoff by leveraging unlabeled data.

==> defs-sciposter.tex <==
\usepackage{hyperref,url}
\usepackage{amsmath,amssymb,amsthm}
\usepackage{tikz}
\usetikzlibrary{fit}
\usepackage{float,graphicx}
\usepackage{stmaryrd,wasysym,clrscode}
\usepackage{etex,etoolbox}
\usepackage{ifthen}
\usetikzlibrary{patterns,positioning}

\newcommand{\Fit}{\mathtt{Fit}}
\newcommand{\DP}{D}
\newcommand{\Subtree}{\operatorname{Subtree}}
\newcommand{\eqdef}{\stackrel{\mathrm{def}}{=}}
\newcommand{\bI}{\mathbb{I}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\sF}{\mathcal{F}}
\newcommand{\sC}{\mathcal{C}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\sB}{\mathcal{B}}
\newcommand{\sI}{\mathcal{I}}
\newcommand{\sP}{\mathcal{P}}
\newcommand{\sX}{\mathcal{X}}
\newcommand{\meet}{\wedge}
\newcommand{\RE}[2]{\operatorname{RE}\left(#1 \ \| \ #2\right)}
\newcommand{\K}{\operatorname{KL}}
\newcommand{\KL}[2]{\operatorname{KL}\left(#1 \ \middle\| \ #2\right)}
\newcommand{\KLs}[3]{\operatorname{KL}_{#1}\left(#2 \ \middle\| \ #3\right)}
\newcommand{\KLm}[2]{\operatorname{KL}_m\left(#1 \ \| \ #2\right)}
\newcommand{\score}[2]{\operatorname{score}\left(#1 \ \| \ #2\right)}
\newcommand{\phih}{\hat{\phi}}
\newcommand{\psih}{\hat{\psi}}
\newcommand{\pw}{\pi}
\newcommand{\B}{B}
\newcommand{\F}{\mathbb{S}}
\newcommand{\bmu}{\mathbb{U}}
\DeclareMathOperator{\loc}{loc}
\DeclareMathOperator{\lub}{lub}
\newcommand{\mloc}{m_{\loc}}
\newcommand{\atom}[1]{#1^{\circ}}
\newcommand{\atoms}[1]{#1^{\circ}}
\newcommand{\stitch}[2]{\overline{#1}^{#2}}
\newcommand{\relaxx}[2]{\widehat{#1}^{#2}}
\DeclareMathOperator{\sn}{sn}
\DeclareMathOperator{\Uniform}{Uniform}
\newtheorem*{theorem}{Theorem}
\newtheorem*{lemma}{Lemma}
\newtheorem*{proposition}{Proposition}
\newtheorem*{corollary}{Corollary}
\newtheorem*{assumption}{Assumption}
\theoremstyle{definition}
\newtheorem*{example}{Example}
\newtheorem*{definition}{Definition}
\newtheorem*{property}{Property}
\DeclareMathOperator{\Geometric}{Geometric}



==> experiments.tex <==
\section{Experiments}
\label{sec:experiments}

\input{figs-sample-sizes}
\pl{better transition - refer to the staircase example}
\pl{actually, I don't really like this structure, and think the experiments would be better off in the staircase section because that provides more cohesion,
and the intuitions can refer to the experiments directly; then this section can be about other experiments on MNIST and CIFAR-10,
which in some sense we haven't even highlighted in the intro, so we should state there what is the point of them, and what's new?
}

We experimentally study how robustness interacts with standard performance \pl{be more precise} as we vary the number of training samples. We simulate training with various sample sizes for the convex example from Section~\ref{sec:convex} and report the standard test MSE of the standard and robust estimators~\refeqns{stest}{robest}. We compare to the the analogous standard and adversarially trained networks (with $\ell_\infty$ perturbations~\citep{madry2018towards}) on \mnist and \cifar~ datasets by subsampling various amounts. We report final test losses here; trends in generalization gap \pl{have we defined this?} are nearly identical supporting our hypothesis the observed difference in standard performance of the two estimators is due to the different convergence speeds. \pl{explain this better} See Appendix~\ref{sec:app-training-details} for more details.

% \setdefaultleftmargin{0.5cm}{}{}{}{}{}
%% \begin{enumerate}
%%     \item \textbf{Convex example from Section~\ref{sec:convex}}: We consider the square loss $\ell(\theta, x, y)= (y - f_\theta(x))^2 $. We fit cubic B-splines~\citep{friedman2001elements} \ar{Fix the citation--year appears twice} by minimizing the penalized square loss on the training set for different values of the regularization parameter $\lambda$. We compute the standard estimator~\eqref{eq:stest} by optimizing the convex objective and the robust estimator~\eqref{eq:robest} by augmenting the dataset with $\bar{T}(\xline)$ and solving the standard objective with this augmented dataset. \ar{Unclear-- you augment with $T(x)$ for $x$ in training set right? Also, we should probably clarify why we augment and how it differs from the max objective. I am leaning towards doing the max actually..} We simulate training data of varying sizes, and report the average and standard deviation over $2000$ instances for small training set size and $25$ instances for large training set size. See Appendix~\ref{app-spline-implementation} for more details.
%% \item \textbf{\cifar and MNIST.} We train $\wrn{40}{2}$~\citep{zagoruyko2016wide} on \cifar, and a small CNN on MNIST. We report the 0-1 standard test loss for both standard and robust training. For robust training, we consider $\ell_\infty$ perturbations of varying $\epsilon$ and perform \emph{adversarial training} using the gradient based approximation to the worst-case perturbation~\citep{madry2018towards}. See Appendix~\refsec{app-training-details} for details.
%% \end{enumerate}

\subsection{Robustness hurts standard performance}
%% We first consider the case where robustness hurts generalization, increasing the test loss
%% of the robust estimator compared to the standard estimator.
\pl{be more precise / consistent with terminology: adversarial (robust) training, standard accuracy}
We see that robustness \pl{really don't like 'robustness' as a term that does things} hurts standard performance in the convex example when the slope $m=1$ and on \cifar.
Figure~\ref{fig:tradeoff} shows the difference in test errors of the two estimators.
% Figure~\ref{fig:tradeoff} shows the difference in test losses
% of the two estimators for the convex example $\distrib(m=1)$ and \cifar where we observe this phenomenon.

When $m=1$, note that fitting the robustness set $B(x)$ requires a more complex solution (See Figure~\ref{fig:schematica}).
With few samples, this complex robust estimator generalizes poorly, leading to high test error (See Figure~\ref{fig:tradeoff-small-sample}).
We sample more from one portion of $\xline$, to exaggerate the poor generalization of the robust estimator on the rest of the support.
\ar{I am not sure if this line is clear..}
In contrast, as the training set mostly contains points from $\xline$~\refeqn{input},
$\stest$ approximates the simple linear estimator that fits $\xline$.
As sample size increases, the complex robust estimator $\robest$ also generalizes well, and the standard test errors of both estimators converge (Figure~\ref{fig:tradeoff-large-sample}).
\pl{all of this really highly overlaps with what should be in the staircase section, explaining the tradeoffs,
another reason to merge}

\pl{need to explain regularization more}
This trend occurs for all regularization parameters $\lambda$.
The largest difference occurs for intermediate $\lambdamed$, where $\lambdamed$ is large enough to cause $\stest$ to be simple, but $\robest$ is complex.
\pl{I don't understand why this should happen or more fundamentally, why does it even make sense to use the same regularization parameter
for both estimators instead of tuning it separately?}

Perhaps even more surprisingly, an estimator trained with data augmentation, where we replace the maximization by an expectation over the robustness set $B(x)$, sees a similar drop in standard performance.
\pl{need to explain why this is surprising; people won't have context}

%% \ar{Should we even say this?}
%% In fact, the robust estimator has \emph{slightly} lower loss for intermediate $n$, because it also fits $T(\xline)$ (edges of the staircase) which have a small but non-zero $\delta$ mass in the underlying distribution.
The trends from the convex example are mirrored in \cifar: adversarially trained models have larger standard test error than the standard trained models with the  difference getting smaller as the sample size $n$ increases. This supports the hypothesis that the \emph{tradeoff} observed in real datasets is due to insufficient samples for good generalization of complex robust estimators. Moreover adding more samples should mitigate this tradeoff---indeed, adding unlabeled samples suffice (see Section~\ref{sec:rst}).
\pl{don't make this a throw-away sentence - this is something to be emphasized, but maybe not here}

\subsection{Robustness helps standard performance}
Robustness can help standard performance in the convex example when the slope $m=0$, mirroring our observations on \mnist. \pl{there seems to be an extra space after \mnist - shouldn't be there for punctuation}
Figure~\ref{fig:tradeon} presents the results for these two settings. 
%% We now consider the cases where robustness helps and the robust estimator $\robest$ has smaller test loss. Figure~\ref{fig:tradeon} presents the results on the convex example $\distrib(m=0)$ (defined in Section~\ref{sec:convex}) and \mnist. In both cases, we see that the robust estimator has lower test loss than the standard estimator.

When $m=0$, the optimal predictor is linear (Figure~\ref{fig:schematicb}).
Since enforcing robustness doesn't increase complexity of the estimator, $\robest$ does not have larger test  error.
% On the other hand, notice that
In fact, by enforcing invariance on $B(x)$, $\robest$ is less sensitive to target noise \pl{defined?} and has \emph{lower} test error (Figure~\ref{fig:tradeon-small-sample}).
This is reflected in the largest gains of $\robest$ over $\stest$ for a small sample size and small $\lambda$ (where $\stest$ overfits to noise).
Both estimators are consistent and the test errors converge as sample size increases.

Similarly, on \mnist, the adversarially trained model has lower test error than standard trained model. As we increase the sample size, both standard and adversarially trained models converge with the same small test error. We remark that our observation on \mnist is contrary to that reported in \citep{tsipras2019robustness}, due to a different initialization that led to better optimization (see Appendix Section~\ref{sec:app-init-mnist}). 
%% For the convex case, we see that for small $n$, $\testloss(\stest(\lambda))$ is larger than $\testloss(\advest(\lambda))$. As $n$ increases, the gap closes. The gap between the estimators depends on the regularization parameter $\lambda$. We see the largest gap for medium $\lambda$, where $\advest(\lambda_\text{medium})$ overfits much more than $\stest(\lambda_\text{medium})$. (b) On subsampling CIFAR-10, we see that the gap between test loss of standard training and test loss of robust training (adversarial training) decreases on increasing the number of samples, just like the convex case in (a). Extrapolating the trend, we see that the gap should close as the number of training of training samples increase.}

